A 334$\mu$W 0.158mm$^2$ ASIC for Post-Quantum Key-Encapsulation Mechanism Saber with Low-latency Striding Toom-Cook Multiplication Authors Version

The hard mathematical problems that assure the security of our current public-key cryptography (RSA, ECC) are broken if and when a quantum computer appears rendering them ineffective for use in the quantum era. Lattice based cryptography is a novel approach to public key cryptography, of which the mathematical investigation (so far) resists attacks from quantum computers. By choosing a module learning with errors (MLWE) algorithm as the next standard, National Institute of Standard & Technology (NIST) follows this approach. The multiplication of polynomials is the central bottleneck in the computation of lattice based cryptography. Because public key cryptography is mostly used to establish common secret keys, focus is on compact area, power and energy budget and to a lesser extent on throughput or latency. While most other work focuses on optimizing number theoretic transform (NTT) based multiplications, in this paper we highly optimize a Toom-Cook based multiplier. We demonstrate that a memory-efficient striding Toom-Cook with lazy interpolation, results in a highly compact, low power implementation, which on top enables a very regular memory access scheme. To demonstrate the efficiency, we integrate this multiplier into a Saber post-quantum accelerator, one of the four NIST finalists. Algorithmic innovation to reduce active memory, timely clock gating and shift-add multiplier has helped to achieve 38% less power than state-of-the art PQC core, 4x less memory, 36.8% reduction in multiplier energy and 118x reduction in active power with respect to state-of-the-art Saber accelerator (not silicon verified). This accelerator consumes 0.158mm2 active area which is lowest reported till date despite process disadvantages of the state-of-the-art designs.

==> source_inputs/biographies.tex <==
%\begin{comment}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/ISCC JPG.jpg}}] {Archisman Ghosh} is a Ph.D. student in Electrical and Computer Engineering at Purdue University, working with Professor Shreyas Sen. He received his Bachelor of Electronics and Telecommunication Engineering from Jadavpur University, India, in 2017. Prior to joining his Ph.D., he worked as a Digital Design \& Verification Engineer at Samsung Semiconductor India R \& D. He interned with the Power Delivery Circuits \& Systems group, Intel Labs, OR, over the summer of 2020. His research interests include mixed-signal IC design and hardware security. He was a recipient of the prestigious SSCS predoctoral achievement award for the year 2022. He is also a recipient of a prestigious ECE fellowship and Bilsland Dissertation Fellowship from Purdue University. He has been serving as a Primary Reviewer for multiple reputed journals and conferences, including IEEE International Conference on VLSI Design (VLSID), Transactions on Circuits \& Systems - II (TCAS-II), and Wireless Personal Communication (WPC) (Springer).
 \end{IEEEbiography}
 \vspace{-1.3cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Jose_converted.jpg}}] {Jose Maria Bermudo Mera} received the Bachelor and Master of Science in Telecommunication Engineering from the Technical University of Madrid in 2014 and 2016, respectively. He worked as research assistant at the Technical University of Munich, Germany, and joined COSIC at KU Leuven, Belgium, in 2017. He obtained a Ph.D. in Electrical Engineering working with Prof.Dr.Ir. Ingrid Verbauwhede and Dr. Angshuman Karmakar. The topic of his thesis was implementation aspects of lattice-based crptography. Since November 2022, Jose works for PQShield Ltd as Cryptography Hardware Design Engineer.
 \end{IEEEbiography}
 \vspace{-1.3cm}
 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Angshuman Karmakar.JPG}}] {Angshuman Karmakar} received a B.E. in computer science and engineering from Jadavpur University, Kolkata, an M.Tech. in computer science and engineering from the Indian Institute of Technology, Kharagpur, and a Ph.D. from Katholieke Universiteit Leuven (KU Leuven), Belgium, for his dissertation titled “Design and Implementation Aspects of Post-Quantum Cryptography.” He is one of the primary designers of the post-quantum Saber KEM scheme which is one of the finalists in the NIST’s post-quantum standardization procedure. He
received FWO Post-Doctoral Fellowship with the COSIC Research Group, KU Leuven. He is currently working as an assistant professor at the department of Computer science and engineering at the Indian Institute of Technology, Kanpur, India. His research interests span different aspects of lattice-based post-quantum cryptography and computation on encrypted data.
 \end{IEEEbiography}
 \vspace{-1.1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/debayan_das.png}}]{Debayan Das} received his PhD and MS in Electrical and Computer Engineering from Purdue
University, USA in 2021, and the Bachelor of Electronics and Telecommunication Engineering degree from Jadavpur University, India, in 2015. He is currently a Research Scientist at Intel Corporation, USA. Prior to his Ph.D., he worked as an Analog Design Engineer at a startup based in India. He has interned with the Security Research Lab, Intel Labs, USA, over the summers of 2018 and 2020. His research interests include mixed-signal IC design and hardware security.
Dr. Das was a recipient of the IEEE HOST Best Student Paper Award in 2017 and 2019, the Third Best Poster Award in IEEE HOST 2018, and the 2nd Best Demo Award in HOST 2020. In 2019, one of his papers was recognized as a Top Pick in Hardware and Embedded Security published over the span of the last six years. He was recognized as the winner (third place) of the ACM ICCAD 2020 Student Research Competition (SRC). During his Ph.D., he has been awarded the ECE Fellowship during 2016–2018, the Bilsland Dissertation Fellowship in 2020–2021, the SSCS Pre-doctoral Achievement Award in 2021, and the Outstanding Graduate Student Research Award by the College of Engineering, Purdue University, in 2021 for his outstanding overall achievements. He has authored/co-authored more than 50 peer-reviewed conferences and journals including 2 book chapters and 2 US patents. He has been
serving as a primary reviewer for multiple reputed journals and conferences including JSSC, TCAS-I, TVLSI, TCAD, Design \& Test, TODAES, JETCAS, TBME, IEEE Access, IoTJ, DAC, VLSI Design, HOST.

\end{IEEEbiography}
%\vspace{-5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/santosh ghosh bio.jpg}}]{Santosh Ghosh} is a Research Scientist in Intel Labs. He has coauthored about 65 research publications in refereed international conferences and journals with a citation H-index of 21, and 20 issued with other 51 more patents filed (pending). The primary focus of his research includes: 1) design and implement cryptographic hardware microarchitecture and RTL with the aggressive area, latency, and throughput constraints; multiple of them are already being deployed in high-volume Intel products; 2) investigate and develop timing, power, and EM side-channel countermeasures; and 3) collaborate with academic partners and provide cryptography and security guidance to Intel business units. Santosh received the Ph.D. degree from IIT Kharagpur, India in 2011, and completed his post-doctoral studies from COSIC, KU Leuven, Leuven, Belgium, in the area of cryptographic hardware and side-channel attacks.
\end{IEEEbiography}
 \vspace{-1.2cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Ingrid.JPG}}]
{Ingrid Verbauwhede} is a professor with the Research Group COSIC, Electrical Engineering Department, KU Leuven. At COSIC, she leads the secure embedded systems and hardware group. She was elected as member of the Royal Flemish Academy of Belgium for science and the arts in 2011. She received the IEEE 2017 Computer Society Technical Achievement Award. She is a recipient of two ERC Advanced Grants, one in 2016 and a second one in 2021.
She is a pioneer in the field of efficient and secure implementations of cryptographic algorithms on many different platforms: ASIC, FPGA, embedded, cloud. With her research, she bridges the gaps between electronics, the mathematics of cryptography, and the security of trusted computing. Her group owns and operates an
advanced electronic security evaluation lab. She received the 2023 IEEE Donald O. Pederson Award. She is a Fellow of IEEE and IACR.
\end{IEEEbiography}
 \vspace{-1.2cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/shreyas_sen.jpg}}]{Shreyas Sen} (S’06–M’11–SM’17) is an Elmore Associate Professor of ECE \& BME, Purdue University and received his Ph.D. degree from ECE, Georgia Tech. Dr. Sen has over 5 years of industry research experience in Intel Labs, Qualcomm and Rambus. His current research interests span mixed-signal circuits/systems and electromagnetics for the Internet of Things (IoT), Biomedical, and Security. He has authored/co-authored 3 book chapters, over 175 journal and conference papers and has over 20 patents granted/pending. Dr. Sen serves as the Director of the Center for Internet of Bodies (C-IoB) at Purdue. Dr. Sen is the inventor of the Electro-Quasistatic Human Body Communication (EQS-HBC), or Body as a Wire technology, for which, he is the recipient of the MIT Technology Review top-10 Indian Inventor Worldwide under 35 (MIT TR35 India) Award in 2018 and Georgia Tech 40 Under 40 Award in 2022. To commercialize this invention Dr. Sen founded Ixana and serves as the Chairman and CTO. His work has been covered by 250+ news releases worldwide, invited appearance on TEDx Indianapolis, Indian National Television CNBC TV18 Young Turks Program, NPR subsidiary Lakeshore Public Radio and the CyberWire podcast. Dr. Sen is a recipient of the NSF CAREER Award 2020, AFOSR Young Investigator Award 2016, NSF CISE CRII Award 2017, Intel Outstanding Researcher Award 2020, Google Faculty Research Award 2017, Purdue CoE Early Career Research Award 2021, Intel Labs Quality Award 2012 for industrywide impact on USB-C type, Intel Ph.D. Fellowship 2010, IEEE Microwave Fellowship 2008, GSRC Margarida Jacome Best Research Award 2007, and nine best paper awards including IEEE CICC 2019, 2021 and in IEEE HOST 2017-2020, for four consecutive years. Dr. Sen's work was chosen as one of the top-10 papers in the Hardware Security field (TopPicks 2019). He serves/has served as an Associate Editor for IEEE Solid-State Circuits Letters (SSC-L), Nature Scientific Reports, Frontiers in Electronics, IEEE Design \& Test, Executive Committee member of IEEE Central Indiana Section and Technical Program Committee member of DAC, CCS, CICC, IMS, DATE, ISLPED, ICCAD, ITC, VLSI Design, among others. Dr. Sen is a Senior Member of IEEE.
\end{IEEEbiography}

%\end{comment}
